Categorified Jones-Wenzl Projectors and Generalizations

This preprint comprises the first four out of five chapters of the Master's thesis I wrote 2022 under the supervision of Catharina Stroppel and Paul Wedrich at the University of Bonn titled "Categorified Jones-Wenzl projectors and Generalizations". Chapter 1 can serve as introductory literature for researchers or graduate students familiar with Schur-Weyl duality between the symmetric group and the general linear Lie algebra or their quantum counter parts, and who are seeking to learn a type B/D analogue of the famous type A story. Chapter 1 serves as an introduction to the type B combinatorics and blob-diagrammatics. Chapters 2,3, and 4 contain proofs of three main theorem each - the first one is an explicit/computational proof of the easiest case of quantum coideal Schur-Weyl duality involving non-trivial quantizations of weight spaces, the second one shows the generalization of Jones-Wenzl projectors to the type B Temperley-Lieb algebra and the third one uses generalized Reidemeister moves and a functional analytic argument to prove a version of the fact that powers of the type D full-twist converge towards the type D Jones-Wenzl projector.

==> MA_Titlepage.tex <==
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{MA_Titelseite}[2010/04/25]

%%%%%%%%%%%%%%%%
% Titelseite:
%%%%%%%%%%%%%%%%
\newcommand*{\betreuer}[1]{\def\@betreuer{#1}}
\betreuer{}
\newcommand*{\zweitgutachter}[1]{\def\@zweitgutachter{#1}}
\zweitgutachter{}
\newcommand*{\ausarbeitungstyp}[1]{\def\@ausarbeitungstyp{#1}}
\ausarbeitungstyp{}
\newcommand*{\geburtsdatum}[1]{\def\@geburtsdatum{#1}}
\geburtsdatum{}
\newcommand*{\geburtsort}[1]{\def\@geburtsort{#1}}
\geburtsort{}
\newcommand*{\institut}[1]{\def\@institut{#1}}
\institut{}

\renewcommand\maketitle{\begin{titlepage}%
  \let\footnotesize\small
  \let\footnoterule\relax
  \let \footnote \thanks
  \null\vfil

\begin{center}%

\parbox{10cm}{\centering\huge\bfseries \@title \par}\\
\vspace{1em}
{\Large
\vspace{1em}
\@authornew}\\
\vspace{1em}
Born \@geburtsdatum \ in \@geburtsort\\
\vspace{1em}
{\large \@date}
\vspace{10em}

{\large \@ausarbeitungstyp}\\
\vspace{1em}
{\large \@betreuer}\\
\vspace{1em}
{\large \@zweitgutachter}\\
\vspace{1em}
\centerline{{\large\scshape \@institut}}
\vspace{10em}

\centerline{{\large\scshape Mathematisch-Naturwissenschaftliche Fakult\"at der}}
\vspace{1em}
\centerline{{\large\scshape Rheinischen Friedrich-Wilhelms-Universit\"at Bonn}}

\end{center}

\vfil\null
\clearpage
\thispagestyle{empty}\mbox{}
\clearpage

\end{titlepage}%

  \setcounter{footnote}{0}%
  \global\let\maketitle\relax
  \global\let\@authornew\@empty
  \global\let\@date\@empty
  \global\let\@title\@empty
  \global\let\title\relax
  \global\let\author\relax
  \global\let\date\relax
  \global\let\and\relax
}
% END Titelseite

\endinput

